Benchmark Dataset Dynamics, Bias and Privacy Challenges in Voice Biometrics Research

Speaker recognition is a widely used voice-based biometric technology with applications in various industries, including banking, education, recruitment, immigration, law enforcement, healthcare, and well-being. However, while dataset evaluations and audits have improved data practices in face recognition and other computer vision tasks, the data practices in speaker recognition have gone largely unquestioned. Our research aims to address this gap by exploring how dataset usage has evolved over time and what implications this has on bias, fairness and privacy in speaker recognition systems. Previous studies have demonstrated the presence of historical, representation, and measurement biases in popular speaker recognition benchmarks. In this paper, we present a longitudinal study of speaker recognition datasets used for training and evaluation from 2012 to 2021. We survey close to 700 papers to investigate community adoption of datasets and changes in usage over a crucial time period where speaker recognition approaches transitioned to the widespread adoption of deep neural networks. Our study identifies the most commonly used datasets in the field, examines their usage patterns, and assesses their attributes that affect bias, fairness, and other ethical concerns. Our findings suggest areas for further research on the ethics and fairness of speaker recognition technology.

==> sections/3_background.tex <==
\section{Background}
\label{s:background}
% 2 pages


% This section contextualizes speaker recognition technology %within the broader field of automatic speech processing and 
% within its historical development. We also show the influence of evaluation-driven research on speaker recognition technology. %A note on terminology: we use the terms \textit{speech} and \textit{voice} interchangeably but adopt wording from the scientific literature whenever possible. While the speech research community clearly distinguishes \textit{voice} and \textit{speech}, people outside the field and in the public domain are less strict about the distinction. 

% \subsection{Automatic Processing of the Human Voice}
% @Wiebke - 0.5 - 0.75 pages

% Table with SR & other voice processing tasks (emotion recognition, identification of demographic attributes, trust factor, etc.) ...can get from interspeech sessions
% Dataset creep (dataset collected for one purpose and use for every possible task)
% Speech technology can be broadly understood as those digital technologies that use automatic speech processing to recognize, characterize, encode or emulate the human voice. Automatic speech processing consists of a variety of domains and tasks, the most important of which are briefly introduced and shown in Figure~\ref{fig:speech_tech_overview}. Speech recognition~\cite{Sen2019AudioOverviews} is perhaps the best known speech processing technology, as automatic speech recognition (ASR, also known as speech-to-text or STT) is integrated into many consumer products like voice assistants and video captioning on conference calls, to transform spoken audio to text. Its generative counterpart, speech synthesis~\cite{Tan2021ASynthesis} (also known as speech generation or text-to-speech (TTS)) simulates the human voice. Speech coding~\cite{Spanias1994SpeechReview} (or speech compression) is concerned with the digital representation of voice signals for efficient transmission and storage. Where speech recognition is concerned with \textit{what was said}, independent of who said it, speaker recognition~\cite{hansen2015speaker, Bai2021Speaker} does the opposite: its aim is to determine \textit{who spoke}, independent of the words that were said. Finally, while speaker recognition aims to identify a person, speaker characterisation~\cite{Schuller2013ParalinguisticsChallenge} (also called paralinguistics), is concerned with identifying attributes of a person, such as their emotional state, gender, age, accent and health. 

% \begin{figure}[hbt]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/speech_tech_overview.jpg}
%     \caption{Contextualising speaker recognition technology within human speech processing.}
%     \label{fig:speech_tech_overview}
% \end{figure}

% \noindent Speaker recognition, which is the application domain studied in this paper, encompasses three main tasks: speaker identification, speaker verification, and speaker diarization~\cite{Bai2021Speaker}. In speaker \textit{identification}, a speaker's identity is determined from a set of known identities. In speaker \textit{verification}, the identity of a speaker is validated against a claimed identity. Speaker \textit{diarization} separates spoken conversations to detect and track who spoke when~\cite{Zheng2017robustness}. Speaker identification and verification are closely related, and systems built for one task can be modified for the other. Models for all three tasks are trained and evaluated on the same datasets. Anti-spoofing and voice privacy are two additional subfields of speaker verification that address the rising security and privacy threats that accompany the wide-scale deployment of speaker recognition technology~\cite{Bonastre2021benchmarking}. 

% Research on bias and fairness is scarce across all domains of speech processing. While this paper focuses on speaker recognition, datasets in speech processing are frequently reused across multiple domains and tasks~\cite{le2014categorization}. The insights we share in this study can thus guide research on bias and fairness in other speech processing domains in the future. 

% \subsection{History of Speaker Recognition Development}

% The development of speaker recognition technology has a rich history dating back to the 1960s and 1970s~\cite{pruzansky1964talker, Furui200550Research, Bai2021Speaker}. The first fully automated speaker recognition system was built by Texas Instruments in the early 1970s and relied on four-word recombinations of 16 trained words for speaker verification~\cite{Doddington1971AVerification, Furui200550Research}. In the 1980s, statistical models, including Hidden Markov Models (HMMs), replaced rule-based speech recognition systems and became the new standard in speaker verification~\cite{Naik1989SpeakerLines}. By the early 1990s, automatic speaker verification was already widely used in security-sensitive industries such as the military and nuclear power plants, as well as for tele-monitoring individuals on probation. At this point, research in automatic speaker recognition was underway, but commercial reliability was still lacking~\cite{Kunzel1994CurrentRecognition}.

% In the mid 1990s to early 2000s, Gaussian Mixture Models (GMMs) in combination with HMMs contributed to advancements in speaker recognition technology. In 1995, Reynolds reported a 99.5\% accuracy on the TIMIT database, 60.7\% on NTIMIT, and 82.8\% on the Switchboard database. Reynolds also noted differences in model performance for male and female speakers, with lower performance for female speakers (99\%, 56.5\%) compared to male speakers (99.8\%, 62.5\%) when the system was trained on a database consisting of 438 males and 192 females speakers~\cite{Reynolds1995Speaker}. This bias was not attributed to the gender imbalance in the training database. 

% By the mid 2010s deep neural networks (DNNs) replaced HMMs and GMMs as the dominant model used for speaker recognition systems due to their overall better performance, and other benefits such as their ability to learn from unlabeled training data~\cite{Hutiri2022BiasRecognition}. Unlike HMMs and GMMs, the performance of DNNs improves with an increasing training set size, provided that the target speaker is well represented in the training set~\cite{Reynolds1995Speaker, Chung2019DelvingRecognition, Khoury2013TheEnvironment}. In speaker recognition, individual speaker voice can be challenging to identify due to variations caused by the channel and speaker. To address this issue, Dehak et al. (2010) introduced a technique of reducing these variabilities through factor analysis, resulting in low-dimensional i-vectors rather than the prior approach of using high-dimensional supervectors~\cite{dehak2010front, Bai2021Speaker}. This transformation helped reduce speaker and channel variations, ultimately enhancing the performance of the speaker recognition system. DNNs in speaker recognition advanced with the introduction of the d-vector embedding technique in 2014. This technique was one of the first to employ a DNN for speaker representation by using the speaker identity of a training utterance as labels for each frame of the utterance~\cite{variani2014deep, Bai2021Speaker}. The next stage in the evolution of speaker recognition models was the advent of the x-vector in 2017~\cite{snyder2017deep,snyder2018x,Bai2021Speaker}. This approach shifted the focus from frame-level speaker labels to utterance-level speaker labels, leveraging an aggregation process for improved accuracy.

% Automatic speaker recognition system's performance is also dependent on whether the speech samples are collected in quiet controlled environments, or environments with background noise or interruptions from other speakers. Large publicly available datasets such as VoxCeleb (released in 2017)~\cite{Bai2021Speaker} use speech samples recorded in noisy or natural environments, allowing for the development of systems that can recognize speech or target speakers despite background noise or interruptions. Most of these databases contain mainly English speech samples. Inspired by VoxCeleb, CN-Celeb, a database of Mandarin speech also collected in noisy or natural environments, was released in 2020~\cite{fan2020cn}. 
% As these speech and speaker recognition systems depend on or coevolve with the datasets used to develop them~\cite{Greenberg2020}, the composition of a systems training dataset can tell us a lot about a system's capabilities, limitations, and intended uses. 

%\medskip \noindent \textbf{Present and Future Applications} \par 
%\noindent Today, speaker recognition is widely used by the public and by public-facing institutions, bringing concerns about biases in these systems and their surveillance applications into public discourse. Banks use speaker identification to verify their customer’s identity~\cite{TDPersonalBankingVoicePolicy, BMOVoiceWorks}, and large companies use them to verify the identity of their employees~\cite{ThomasHeath2016ThisBathroom}. Several companies in the United States have used or looked into using speaker recognition and other surveillance techniques to ‘monitor worker emotions to boost performance and compliance’~\cite{Kinni2016MonitoringIndustry}. As the applications of these systems continue to expand and become more essential to public life, underrepresented speakers may be misidentified, and face unjust barriers to or exclusion from participating in public life. Automatic speaker recognition systems also pose a threat to citizens privacy. Speaker identification has provided governments a relatively low-cost method to drastically increase their surveillance capabilities and reach. The Chinese Government’s use of speaker recognition technologies for surveillance have served as a cautionary tale. Speaker identification is routinely used to identify speakers on private phone calls, and in some regions providing speech samples have become a requirement to obtain a passport~\cite{Qiang2019PresidentState}. %Siri and Alexa’s speech recognition accuracy's have been shown to be about 20\% lower for individuals with voice disorders - about 1 in 13 adults in America today~\cite{Rohlfing2021}.

% can we get the details for this table from~\cite{Bai2021Speaker}?
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|cccc}
%          \textbf{Period} & \textbf{Dominant Datasets} & \textbf{Dominant Models} & \textbf{Applications} & \textbf{Funders}\\ \midrule
%          1996 - 2003 & Switchboard & GMMs &  & \\
%          2004 - 2011 & Switchboard, Mixer & HMM/GMMs &  & \\
%          2012 - 2017 & Switchboard, Mixer & i-vector &  & \\
%          2018 - 2021 & VoxCeleb & Deep Neural Networks (x-vector) &  & \\
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}


% \subsection{Evaluation-driven Development of Speaker Recognition Technology} \label{ss:NIST}
The advancement of speaker recognition technology has been greatly influenced by evaluation-driven research.  For over two decades, the National Institute of Standards and Technology (NIST) has been conducting Speaker Recognition Evaluations (SREs) to evaluate and improve current speaker recognition technology~\cite{Greenberg2020}. To support these evaluations, NIST collected and split speech corpora into development and evaluation sets. NIST aimed to collect data from speakers with different demographics, in multiple languages, and with varying vocal effort levels. A summary of the speaker recognition challenges, the corresponding development datasets and tasks is presented in Table~\ref{tab:SRC-overview}. 

\begin{table*}[hbt]
\small
\renewcommand{\arraystretch}{1.05}
% \resizebox{\linewidth}{!}{
\begin{tabular}{L{0.25\linewidth}|c|L{0.2\linewidth}|L{0.25\linewidth}|C{0.08\linewidth}}
\textbf{SRC name} & \textbf{Year} & \textbf{Speaker Recognition Task} & \textbf{Development Data} & \textbf{Add. Dev. Data}\\ \midrule
NIST SRE Phase I \cite{NISTEvalPlan1997, NISTEvalPlan1998, Martin2001The1996-2001, NISTEvalPlan1999, NISTEvalPlan2000, NISTEvalPlan2001, NISTEvalPlan2002, NISTEvalPlan2003} & 1996 - 2003 & Detection, Tracking, Segmentation &  Switchboard, CALLHOME, FBI Voice Dataset & \xmark \\ \midrule
NIST SRE Phase II \cite{NISTEvalPlan2004, NISTEvalPlan2005, NISTEvalPlan2006, NISTEvalPlan2008, NISTEvalPlan2010, NISTEvalPlan2012} & 2004 - 2012 & Detection, Human-Assisted SR (2012) &  Switchboard, Mixer & \checkmark \\
SRE in Mobile Env's \cite{Khoury2013TheEnvironment} & 2013 & Verification & MOBIO & \checkmark\\ \midrule
ASVspoof~\cite{ASVSpoof2015,ASVSpoof2017,ASVSpoof2019,ASVSpoof2021} & 2015 - ongoing & Spoofing Countermeasures & SASCorpus, RedDots, VCTK, ASVSpoof database & \checkmark \footnote{until 2017} \\
NIST SRE Phase III \cite{NISTEvalPlan2016, NISTEvalPlan2018, NISTEvalPlan2019, NISTEvalPlan2021} & 2016 - ongoing & Detection & Switchboard, Mixer, Fisher, Call My Net, JANUS Multimedia, VoxCeleb & \checkmark \\
Speakers in the Wild SRC \cite{mclaren2016speakers} & 2016 & Detection & SITW Database & \checkmark\\
VoxCeleb SRC \cite{Nagrani2020Voxsrc} & 2019 - 2021 & Verification, Diarisation & VoxCeleb & \checkmark \\
Far-Field SVC \cite{Qin2020TheChallenge} & 2020, 2022 & Far-Field Verification & DMASH, FFSVC Database, HI-MIA & \checkmark \footnote{as long as publicly and freely available on \url{http://openslr.org/}}\\
Short Duration SVC \cite{zeinali2019shortduration} & 2020 - 2021 & Verification & DeepMine, VoxCeleb, LibriSpeech & \xmark \\
Speech Processing Universal Performance Benchmark (SUPERB) \cite{yang2021superb} & 2021 - ongoing & Identification, Verification, Diarisation & VoxCeleb, LibriMix & \xmark \\
CN-Celeb SRC \cite{CNCELEBEvalPlan} & 2022 & Verification, Retrieval & CN-Celeb & \checkmark \\
\end{tabular}
\caption{Overview of Speaker Recognition Challenges (SRCs). The right column indicates whether additional training data was permitted.}
\label{tab:SRC-overview}
\end{table*}

The utilization of datasets in evaluation tasks has undergone three phases. From 1996 to 2003, the SREs relied on the various Switchboard corpora. The SRE 2004 introduced the Mixer corpus and the recruitment of bilingual speakers, allowing for the evaluation of language's influence on speaker recognition performance~\cite{Gonzalez-Rodriguez2014}. During NIST SRE Phase II, participants were allowed to use additional speech corpora for development, as long as they were described in the system descriptions\cite{NISTEvalPlan2004}. This phase involved combining and remixing previously collected datsets, with caution advised due to the risk of bias and case duplications. NIST evaluations warned of these risks, but researchers reusing NIST datasets may not be aware of overlapping speakers. For instance, NIST allowed the usage of the original Switchboard-1 corpus in 2004, but warned that speakers from this corpus may reappear in the evaluation dataset~\cite{NISTEvalPlan2004}.

The NIST SREs have implemented fixed and open conditions for development datasets since 2016.~\cite{Greenberg2020}. Fixed training conditions enable meaningful comparisons of systems, while open conditions allow for exploration of promising research with unrestricted data usage~\cite{Greenberg2020}. Challenges like VoxCeleb SRC and CN-Celeb SRC use both conditions, while others like Short Duration SVC rely solely on fixed conditions. 

% I changed the order of the subsections here. As discussed, I thought it would be helpful to merge 3.3 and the Results Section on NIST. This could allow us to discuss the dynamics of datasets within the NIST SRE challenges but also across different challenges. For example, we can see from the Table that recently developed challenges rely mostly on open-source datasets such as VoxCeleb while NIST still tries to make an effort to collect datasets for specific task conditions.

%\subsection{Evaluation-driven advances in speaker recognition technology}
% @Wiebke

%\begin{table}[hbt]
%\begin{tabular}{p{0.3\linewidth}|c|p{0.3\linewidth}|p{0.2\linewidth}}
%\textbf{SRC name} & \textbf{Year} & \textbf{Task} & \textbf{Training Datasets} \\
%NIST SRE Phase I \cite{NISTEvalPlan1996, NISTEvalPlan1997, NISTEvalPlan1998, NISTEvalPlan1999, NISTEvalPlan2000, NISTEvalPlan2001, NISTEvalPlan2002, NISTEvalPlan2003} & 1996 - 2003 & Speaker Detection \& Speaker Tracking \& Speaker Segmentation &  Switchboard \& CALLHOME \& FBI Voice Dataset \\
%NIST SRE Phase II \cite{NISTEvalPlan2004, NISTEvalPlan2005, NISTEvalPlan2006, NISTEvalPlan2008, NISTEvalPlan2010, NISTEvalPlan2012} & 2004 - 2012 & Speaker Detection \& Human-Assisted Speaker Recognition (2012) &  Switchboard \& Mixer \\
%SRE in Mobile Env's \cite{Khoury2013TheEnvironment} & 2013 & Speaker Verification & MOBIO \\
%NIST SRE Phase III \cite{NISTEvalPlan2016, NISTEvalPlan2018, NISTEvalPlan2019, NISTEvalPlan2021} & 2016 - ongoing & Speaker Detection & Switchboard \& Mixer \& Fisher \& Call My Net \& JANUS Multimedia \& VoxCeleb \& Open Condition\\
%Speakers in the Wild SRC \cite{mclaren2016speakers} & 2016 & Speaker Detection & SITW Database \\
%VoxCeleb SRC \cite{Nagrani2020Voxsrc} & 2019 - 2021 & Speaker Verification \& Speaker Diarisation & VoxCeleb \& Open Condition \\
%Far-Field SVC \cite{qin2020interspeech} & 2020, 2022 & far-field distributed microphone arrays under noisy conditions in real scenes & DMASH \& VoxCeleb \\
%Short Duration SVC \cite{zeinali2019shortduration} & 2020 - 2021 & Speaker Verification & DeepMine \& VoxCeleb \& LibriSpeech \\
%Speech Processing Universal Performance Benchmark (SUPERB) \cite{yang2021superb} & 2021 - ongoing & Speaker Identification \& Automatic Speaker Verification \& Speaker Diarization & VoxCeleb \& LibriMix\\
%CN-Celeb SRC \cite{} & 2022 & Speaker Verification \& Speaker Retrieval & CN-Celeb \& Open Condition \\
%\end{tabular}
%\caption{For SUPERB we consider only the relevant Speaker Recognition Tasks}
%\label{tab:my-table}
%\end{table}

%For over 20 years the National Institute of Standards and Technology (NIST) has been conducting Speaker Recognition Evaluations (SREs) to improve and benchmark current speaker recognition technology~\cite{Greenberg2020}. To allow for this evaluation-driven research, it has been necessary to design, develop and collect new speech corpora and to split them into appropriate development and evaluation sets. Regarding the usage of datasets for the evaluation tasks, three phases can be identified. From 1996 to 2003, the SREs mostly relied on the various Switchboard corpora collected during these times (see Section~\ref{} for detailed information on Switchboard). With the release of the first Mixer corpus and the recruitment of bilingual speakers, the SRE 2004 was the first to allow evaluation of the influence of language on speaker recognition performance~\cite{Gonzalez-Rodriguez2014}. As the Mixer corpora evolved, the SREs continuously updated their development and evaluation sets accordingly (see Section~\ref{} for detailed information on Mixer). Until 2012, the data allowed for the development of speaker recognition systems was clearly defined in the evaluation guidelines. However, in the SRE 2016, NIST introduced a fixed condition, i.e. limited development datasets, and an open condition, i.e. no limitations on the development datasets~\cite{Greenberg2020}. 
%While the fixed training conditions allow for meaningful systems comparison, the open condition allows the exploration of promising research directions and achievable benefits of unrestricted data usage~\cite{Greenberg2020}. 


% FFSVC objectives: 1) benchmark the current speech verification technology under this challenging condition, 2) promote the development of new ideas and technologies in speaker verification, 3) provide an open, free, and large scale speech database to the community that exhibits the far-field characteristics in real scenes.
